Auctions without commitment in the auto-bidding world

Advertisers in online ad auctions are increasingly using auto-bidding mechanisms to bid into auctions instead of directly bidding their value manually. One prominent auto-bidding format is the target cost-per-acquisition (tCPA) which maximizes the volume of conversions subject to a return-of-investment constraint. From an auction theoretic perspective however, this trend seems to go against foundational results that postulate that for profit-maximizing bidders, it is optimal to use a classic bidding system like marginal CPA (mCPA) bidding rather than using strategies like tCPA. In this paper we rationalize the adoption of such seemingly sub-optimal bidding within the canonical quasi-linear framework. The crux of the argument lies in the notion of commitment. We consider a multi-stage game where first the auctioneer declares the auction rules; then bidders select either the tCPA or mCPA bidding format and then, if the auctioneer lacks commitment, it can revisit the rules of the auction (e.g., may readjust reserve prices depending on the observed bids). Our main result is that so long as a bidder believes that the auctioneer lacks commitment to follow the rule of the declared auction then the bidder will make a higher profit by choosing the tCPA format over the mCPA format. We then explore the commitment consequences for the auctioneer. In a simplified version of the model where there is only one bidder, we show that the tCPA subgame admits a credible equilibrium while the mCPA format does not. That is, when the bidder chooses the tCPA format the auctioneer can credibly implement the auction rules announced at the beginning of the game. We also show that, under some mild conditions, the auctioneer's revenue is larger when the bidder uses the tCPA format rather than mCPA. We further quantify the value for the auctioneer to be able to commit to the declared auction rules.

==> dummie.tex <==
\begin{proof}
{\color{red} For the proof we denote by $\underline v, \overline v$ the lowest and upper elements in the support of $F$.

From the revelation principle, without loss of generality we restrict to incentive compatible mechanisms $(\chi,\tau)$ where the bidder receives queries $\{p_0(x)\leq \chi(v)\}$ for a price $\tau(v)$. 

The incentive compatible condition on the mechanism implies that the bidder's utility satisfies that 
$$ vH(\chi (v)) - \tau(v) = \max_{v'} vH(\chi  \chi(v')) - \tau(v').$$

Using the envelope approach \citep{milg02}, we have that the incentive compatibility restriction is equivalent to (i) $\chi (v)$ being non-decreasing (since $H$ is increasing) and (ii) that for almost every type $v$ we have that 
$$\tau T(v) = vH(\chi (v)) - \int_{\underline v}^v H(\chi (z))dz \qquad \mbox{ (IC)}.$$


The previous characterization of $\tau$ allow us to reformulate the auctioneer's revenue as
$$\int_{\underline v}^{\overline v} \left(vH(\chi (v)) - \int_{\underline v}^v H(\chi (z))dz\right) f(v)dv = \int_{\underline v}^{\overline v} \phi_F(v) H(\chi (v)) f(v)dv,$$
where the equality comes from using integration by parts.\footnote{The integrability condition on $H$ (Assumption~\ref{ass:0}) ensures that the integration by parts can be taken for the case where the support of the distribution $F$ is unbounded.}

The intrinsic price condition imposes that the auctioneer receives a payment for at least the intrinsic price of the queries allocated to the bidder. Thus, $\tau(v)\geq \int_{0}^{\chi (v)}zh(z)dz$. We assert that without loss of generality, we can restrict to transfer rules satisfying that for every valuation-types $v_1>v_2$,
$$ \tau(v_1)- \tau(v_2) \geq \int_{\chi(v_2)}^{\chi(v_1)}zh(z)dz \qquad \mbox{ (FC)}.$$
Consider a feasible mechanism $(\chi,\tau)$ such that for some $v_1,v_2$ such that $(FC)$ is not satisfied. Define the {\em improving} transfer rule 
$$\hat \tau (v)= \begin{cases}
\tau(v) &\mbox{ if } v< v_2 \mbox{ or} v > v_1 //
\max\{\tau(v), \tau(v_1)+\int_{\chi(v_2)}^{\chi(v)}zh(z)dz \} &\mbox{ if } v\in [v_2,v_1]
\end{cases}.$$
We claim that the mechanism $(\chi,\hat \tau)$ is also incentive compatible. Indeed, for type a $v<v_2 \mbox{ or} v > v_1$ there is no incentive to deviate as their utility does not change and deviations are less profitable. The same reasoning applies for a type $v\in [v_1,v_2]$ such that $\tau(v)=\hat \tau(v)$. For a type $v$ such that $\tau(v)\neq \hat \tau(v)$, suppose that she prefers to deviate to report a type $v'<v$ with $v'\geq  v_2$. If 
d clearly, 


for every query, the price which is sold has to be at least \amnote{is it ``exactly" in this model?} the respective intrinsic price. This, in terms of $H$, implies that for every feasible transfer rule $T$ and every valuation-types $v>v'$ the following inequality holds:
$$ \tau(v)- \tau(v') \geq \int_{ \chi(v')}^{ \chi(v)}zh(z)dz \qquad \mbox{ (FC)}.$$

We claim that if $x$ satisfies the incentive-compatibility constraint \amnote{(IC)}and the feasibility constraint (FC) then, up to a zero-measure set of types, $ \chi(v)\leq v$. To see this, since $x$ is non-decreasing then is differentiable almost everywhere (see Theorem 7.20 \cite{rudin}). Consequently, $T$ is also differentiable almost everywhere. The (IC) condition implies that $T'(v) = vh( \chi(v))x'(v)$, while the (FC) condition implies that $T'(v) \geq  \chi(v) h( \chi(v))x'(v)$. We conclude that $ \chi(v)\leq v$ for almost every valuation type $v$.    

To conclude the proof, consider the following relaxation of the auctioneer's problem 
\begin{align*}
    \max_{ \chi(\cdot)}\quad &\E_v \left[H( \chi(v)) \;\phi_F(v)\right] \\
    \mbox{s.t. }\quad &  \chi(v)\leq v \quad (a.e.).
\end{align*}

Because $H$ is increasing and $\phi_F$ is increasing, the above problem admits a pointwise solution which is 
$$ x^*(v)= \begin{cases}
0 &\mbox{ if } v < r_{\mye} \\
v &\mbox{ if } v\geq r_{\mye}
\end{cases}.
$$

We conclude the proof by showing that $x^*$ is solution for the auctioneer's problem. Indeed, first observe that $x^*$ is monotone, and hence, $x^*$ satisfies condition (i) in the incentive-compatibility restriction. Moreover, the transfer rule generated by $x^*$ is such that for $v\geq r_{\mye}$,
$$T^*(v) = vH(v) - \int_{r_{\mye}}^v H(z)dz = r_{\mye} H(r_{\mye}) +\int_{r_{\mye}}^v z h(z)dz, $$
where we use integration by parts for the second equality. Clearly, $T^*$ satisfies the feasibility constraint (FC). We conclude that $x^*$ is a feasible solution for the auctioneer's problem, and therefore, $(x^*,T^*)$ is the revenue-maximizing mechanism. }
\end{proof}


==> extension.tex <==
\section{Extension: One bidder and multiple unconstrainted bidders}
\label{sec:extension}
\amnote{Move to appendix and point from Sec 3 in a paragraph.}
The goal of this section is to show the robustness of the results about the revenue of platform obtained in Section~\ref{sec:3}. Once again we consider a stylized model to make it tractable and show similar results when there is one bidder bidding in the platform and unconstrained buyers bidding in the queries. The remaining buyers are such that for query $x$ the highest bid is given by $p_0(x)$ while the second highest bid is given by $\beta p_0(x)$ with $\beta<1$.


\begin{lemma}
In any equilibrium of the UA, there exists $v_H$ such that if $b\leq v_H$, the auctioneer sets a reserve price $r_H= \phi_H^{-1}(0)$ and no queries are allocated to ql-bidder. And if $b>v_H$, the auctioneer sets a reserve price $b$.
\end{lemma}

\begin{proof}

Either the auctioneer allocates queries to the ql-bidder or not. If he does, the optimal reserve price $r_H$. Hence, thelet $v_H$ such that 
$$ v_H H(\frac {v_H}  \beta ) + \beta\int_{\frac {v_H}  \beta}^{\infty} zh(z)dz = r_H(H(\frac{r_H}\beta)- H(r_H)) + \beta \int_{\frac{r_H}{\beta}}^\infty zh(z)dz.$$ 

The monotonocity of $H$, implies that $v_H$ is uniquely defined.
\end{proof}

Observe that the previous lemma implies that is from the ql-bidder perspective if his valuation $v<v_H$ it is not worth for him to participate in the auction. On the other hand, if his valuation is $v>v_H$ his decision problem is the same as in the Model I case, with the constraint that $b\ge v_H$.
\begin{proposition}
In every equilibrium of the UA, let $^*b(v)$ the optimal bidding strategies is $b^*(v) = 0$ if $v\le v_H$ and solves
$$ \max_{b\geq v_H} (v-b)H(b),$$
for $v\geq v_H$.
Moreover, let $b(v)$ the solution to Equation~\eqref{eq:1}, then 
$$ b^*(v) = \begin{cases}
0 &\mbox{ if } v\leq v_H\\
v_H &\mbox{ if } v \in (v_H, b^{-1}(v_H))\\
b(v) &\mbox{ if } v> b^{-1}(v_H)
\end{cases}.$$

\end{proposition}

To tackle the TCPA observe that from the auctioneer's perspective, the highest bid he could implicitly dervie from ql-bidder bidding $T$ is $n(T|0)$. Thus, if $n(T|0)\leq v_H$, then ql-bidder is not considered in the auction. Let $T_H$ the unique solution to $n(T_H|0)= v_H$.

Given a bid $T$, the auctioneer's problem consists on solving 
$$\max_{r\in [0,T] }\;  TH(n(r|T)) + n(r|T)\left (H(\frac {n(r|T)}{\beta}) - H(n(r|T))\right) + \beta \int_{\frac {n(r|T)}{\beta}}^\infty zh(z)dz.$$

Given the one to one mapping between $r$ and $n(r|T)$, the above problem is equivalent to solving

$$ \max_{n'\in [T, n(0|T)]} H(n') + n'\left (H(\frac {n'}{\beta}) - H(n')\right) + \beta \int_{\frac {n'}{\beta}}^\infty zh(z)dz.$$

The first order conditions implies that the optimal solution $n^*(T)=n(r^*(T)|T)$ solves that $n^*=\phi_H(T)$. In particular, when $\beta<1$, we have that $\phi_H(v)<v$, which means that $n^*= T$ it is never a solution to the auctioneer's problem.

%For $T<v_H$, the auctioneer's problem consists of solving WRONG
%$$\max_{r\geq 0} n(T|r) H(\frac {n(T|r)} {\beta} ) +\beta \int_{\frac {n(T|r)} {\beta}}^\infty z h(z)dz.$$
%This is equivalent to 
%$$\max_{n \in [\alpha(T), T]} n H(\frac n \beta) + \beta \int_{\frac n \beta}^\infty z h(z)dz.$$
